Measurements of cosmic-ray secondary nuclei at high energies with the first flight of the CREAM balloon-borne experiment

We present new measurements of heavy cosmic-ray nuclei at high energies per- formed during the first flight of the balloon-borne cosmic-ray experiment CREAM (Cosmic-Ray Energetics And Mass). This instrument uses multiple charge detectors and a transition radiation detector to provide the first high accuracy measurements of the relative abundances of elements from boron to oxygen up to energies around 1 TeV/n. The data agree with previous measurements at lower energies and show a relatively steep decline (~E$^-0.6$ to E$^-0.5$) at high energies. They further show the source abundance of nitrogen relative to oxygen is ~10% in the TeV/n region.

==> creamfigs.tex <==

\begin{figure}[p]
% figure 1
  \centering
  \includegraphics[width=0.95\linewidth]{Detector_Schematic.eps}
  \caption{A Schematic view of the CREAM instrument for the first flight.}
  \label{fig:Schematic}
\end{figure}

\begin{figure}[p]
  \centering
  \includegraphics[width=0.95\linewidth]{scatters.eps}
  \caption{Scatter plots for CREAM detectors for a small fraction of the flight data.
Left: The square root of the path-length and gain corrected TCD signal versus the square root of the path-length and gain corrected
CD, also shown are representative cuts applied to select relativistic nuclei (between dashed lines), the vertical units have been
adjusted to be close to the nuclear charge, Z. The event groups for Be(Z=4), B(Z=5), C(Z=6), N(Z=7), and O(Z=7) are clearly visible.
Right: The square root of the corrected TCD signal versus the square root of the corrected SCD for the selected relativistic nuclei
shown on the left panel. Also shown are representative cuts used to select nuclei which do not interact in the instrument (dashed
lines).} \label{fig:Scatters}
\end{figure}

\begin{figure}[p]
  \centering
  \includegraphics[width=0.90\linewidth]{charge.eps}
  \caption{The distribution of the average of the sum of the square root of the corrected TCD signal and the square root of the corrected SCD signal is shown
  for the data cuts of Figure \ref{fig:Scatters} for the Hi-Z triggers during flight. The left hand panel has a linear count scale, the right hand shows the same data with a
  logarithmic vertical scale. This distribution demonstrates the relativistic particle charge resolution which has value of $\sigma_z$=0.16 charge units at Carbon.}\label{fig:Charge}
\end{figure}

\begin{figure}[p]
  \centering
  \includegraphics[width=0.90\linewidth]{trdxy.eps}
  \caption{Left: A typical Oxygen nucleus event in the TRD, both the xz and yz track views are shown superposed. The large circles represent the amplitude of the signal in the proportional
  tube, the lines are the results of the first level track fit. Right: The percentage difference between the TRD signal determined from the xz track and the yz track for oxygen nuclei
  from the flight data. This has an rms value of $\sim$14\%, implying a resolution for the combination of the sum of both views $\sim$7\%. }\label{fig:TRDxy}
\end{figure}

\begin{figure}[p]
  \centering
  \includegraphics[width=0.90\linewidth]{trd-resp-res.eps}
  \caption{The total TRD signal distribution for oxygen nuclei in the flight data selected to be at minimum ionization using the CD.
  The rms resolution is $\sigma\sim $10\%. The response of the TRD with particle energy (GeV/n) for heavy nuclei. The many symbols are from a GEANT4 simulation
  of this response which have been verifies by direct accelerator measurements shown as the large symbols, this is discussed further in\cite{2003ICRC....4.2233S}. Also shown is the expected energy
   resolution for a signal fluctuations distribution with characteristics as shown on the left. At $\sigma$=10\% this gives a resolution in Log$_{10}$(GeV/n) of
   $\sigma$=0.2. Providing an energy resolution $\Delta E/E\sim$60\%.}\label{fig:TRDresp}
\end{figure}



\begin{figure}[p]
  \centering
  \includegraphics[width=0.90\linewidth]{cer-int.eps}
  \caption{Left:The distribution of observed Cerenkov size from oxygen events in the CD for events selected in the TRD to be between a signal size of 115 and 125
  on the response curve shown in Figure \ref{fig:TRDresp} and selected in the charge detectors to be consistent with a relativistic nuclei signal
  as discussed in the text. The two populations are; on the right real high energy events near 100GeV/n and on the left a tail of low energy events near
  400MeV/n which have passed the other selection cuts. The Cerenkov signal can clearly discriminate between these two populations. In the flight analysis this
   distribution is cut to select only events above the signal level of 1.05. Right: The distribution of charge signals measured by the TCD scintillators for
   relativistic nuclei with a cut on the largest SCD pixel signal ($\pm \Delta$Z=0.2) which selects Boron, Z=5, signal. Several of the nuclei enter
   the instrument as a larger charge and undergo spallation in the instrument which produces a Boron nucleus in the SCD charge measurement}\label{fig:Cercut}
\end{figure}

\begin{figure}[p]
  \centering
  \includegraphics[width=1.00\linewidth]{fourway.eps}
  \caption{The results of measurements of ratios of nuclei as a function of energy. Top left: Filled circles show the ratio of Boron to Carbon of this measurement
  with energy after corrections. The horizontal errors are an estimate of the systematic errors in the overall energy scale. The thin vertical lines correspond to the
  statistical error of the ratio. The thick vertical lines show the systematic uncertainty in the ratio, these are dominated at high energy by uncertainties in the correction
  for locally produced Boron nuclei in the atmospheric overburden as discussed in the text. The lines represent model calculations for various values of
  the magnetic rigidity dependence parameter, $\delta$, in escape from the Galaxy as discussed in the text. These are; solid line $\delta$=0.6, long dashed line $\delta$=0.333,
  short dashed line $\delta$=0.7. The stars are data from the space experiment, HEAO-3-C2, which made a high statistics measurement of this ratio at lower energies.
  Top right: Filled circles show the ratio of Nitrogen to Oxygen of this measurement with energy after corrections, error lines and stars have a similar meaning to B/C.
  The lines represent model calculations of this ratio
  with an energy dependent escape parameter $\delta$=0.6 (solid line in the top left hand panel). The different curves correspond to different assumptions on the
  amount of nitrogen in the source material. These are; solid line source N/O = 10\%, long dashed line source N/O = 5\%, short dashed line N/O = 15\%.
  Bottom left: Filled circles show the ratio of Carbon to Oxygen of this measurement with energy after corrections.
  Bottom right: The fluxes (energy/n$\times$area$\times$time$\times$solid angle)$-1$ (arb. units) of Carbon nuclei (open triangles) and
  Oxygen nuclei (open circles) from this measurement. The data is well fit by the dashed line, a power law $\propto$(Energy/n)$^{-\alpha}$ with a spectral index
  $\alpha$=2.6.
    }\label{fig:ratios}
\end{figure}

